Perspectives on Large Language Models for Relevance Judgment

When asked, large language models (LLMs) like ChatGPT claim that they can assist with relevance judgments but it is not clear whether automated judgments can reliably be used in evaluations of retrieval systems. In this perspectives paper, we discuss possible ways for LLMs to support relevance judgments along with concerns and issues that arise. We devise a human--machine collaboration spectrum that allows to categorize different relevance judgment strategies, based on how much humans rely on machines. For the extreme point of "fully automated judgments", we further include a pilot experiment on whether LLM-based relevance judgments correlate with judgments from trained human assessors. We conclude the paper by providing opposing perspectives for and against the use of~LLMs for automatic relevance judgments, and a compromise perspective, informed by our analyses of the literature, our preliminary experimental evidence, and our experience as IR researchers.

==> body/contribution.tex <==
\section{Left-overs}

\ld{This text is a victim of my reorganization. I picked up thoughts not already discussed elsewhere and merged them in the text above. Please double check if I was missing something important}

\subsection{Using LLMs to Generate Annotations and Label Automatically}

\ld{The way the text is currently written, it would fit better in the Introduction. It would help to first introduce the spectrum, then we can refer to it across related work, experiments, future, and conclusion }

Potential uses of LLMs to annotate documents, extract snippets, summarize and, in the end, annotate documents for relevance. If this can be made to work reliably, it opens up many opportunities for evaluation. For example, the LLM can be used directly to evaluate the output of other large language models (for example in summarization). 

Assessments can arise from different sources, with different levels of quality and collection costs as follows. 

\begin{itemize}
    \item Human assessors or, in the enterprise scenario, final users. This scenario, at the current time, is the most expansive, but also likely to produce high-quality annotations.
    \item Human assessors aided by mild automatic support systems (e.g. remove redundancy, encourage consistency)
    \item Half of the judgments are produced by human assessors and half of the judgments are produced automatically.
    \item Automatic annotation of a collection, which is verified and corrected by human intervention.
    \item At some point even a fully automatic assessment.
\end{itemize}


An additional axis describes the type of annotations. Typically an annotation is a graded relevance judgment, but for example in EXAM \cite{sander2021exam}, humans are used for generating questions instead. This can be generalized by asking human assessors for something different than traditional annotation while some Machine Learning (ML) converts the human responses into relevance assessments. This follows the paradigm of Competence Partitioning of Human-Machine-Collaboration where humans and machines are performing tasks they are best at (not vice versa).

\ld{moved to dangers} One concern is that fully automatic assessment with LLMs can be very expensive, which is also the reason why we consider the application of LLMs as part of the retrieval process. In such a case, we could reduce the cost by considering a teacher-student training paradigm (knowledge distillation) in which a large and expensive LLM is used to train a smaller model that is less expensive to run.

\ld{the truth part is moved to dangers} Not all IR tasks focus on topics. For example, one may want to search for podcasts where two or more people interact or with a particular style.
Another issue is regarding truth. For example, finding a podcast for the query “does lemon cure cancer?” that talks about healing cancer with lemon might be on topic. Nevertheless, it is unlikely to be factually correct, and therefore not relevant to correctly answering the information need. To overcome this issue, assessors have to access external information to determine the trustworthiness of a source, or the truthfulness of a document.
In a similar way, we can assume our LLM is used as an oracle that accesses external facts, verified by humans. To properly support different tasks, human intervention can be plugged into the collection and annotation of additional facts, to define relevance.

\ld{moved to dangers} There are open questions for the special case of 100\%-machine / 0\%human. How is this ranking evaluation different from being an approach that produces a ranking? (circularity problem).
We can use multiple LLMs, possibly based on different rationales, such that it is possible to define an inter-annotation systems agreement, in which different systems are used to verify if there is an agreement between each other. An alternative approach is to endow the evaluation with additional information about relevant facts/questions/nuggets that the system (under evaluation) does not have access to. 

\ld{moved to dangers}It is yet to be understood what are the risks associated with such technology: it is likely that in the next few years, we will assist in a substantial increase in the usage of LLMs to replace human annotators. Nevertheless, a similar change in terms of data collection paradigm was observed with the increased use of crowd assessor. Up to that moment, annotations were typically made by in-house experts. Then, such annotation tasks were delegated to crowd workers, with a substantial decrease in terms of quality of the annotation, compensated by a huge increase in annotated data. 
It is a concern that machine-annotated assessments might degrade the quality, while dramatically increasing the number of annotations available.

\ld{merged to dangers} The Cranfield paradigm~\cite{Voorhees2001} is based on simplifying assumptions that make manual evaluation feasible: \textit{1)} independence of queries; \textit{2)} independence of relevance of documents; \textit{3)} Relevance is static (and not changing in time). 
Recently, the field is diverging from this paradigm, for example with TREC CAR and TREC CAST/iKAT where the information needs are developing as the user learns more about the domain. The TREC Evaluation of CAST describes a tree of connected information needs, where one conversation takes a path through the tree. The Human-Machine evaluation paradigm might make it feasible to assess more connected (and hence, realistic) definitions of relevance.


\gd{possibly here or at the end of section 2, it would be good to compare the different methods to collect judgments by their \$ cost, e.g., cost of \$0.05 for an AI to judge;  \$0.50 for the crowd; \$5.00 for NIST assessors?}

==> body/related-work.tex <==
\section{Background and Related Work (max 1.5 pages)}

\label{subsubsec:evaluation-gaps}

\input{body/related-work/rw-human-assessment.tex}
\input{body/related-work/rw-crowd-hybrid-assessment.tex}
\input{body/related-work/rw-automatic-evaluation.tex}
\input{body/related-work/rw-automatic-assessment.tex}

\input{body/related-work/rw-automatic-assessment-LD.tex}

\progressMarker{End of page 5}


==> body/related-work/rw-automatic-assessment-LD.tex <==


\subsection{Automatic Test Collections \ld{already merged into the new RW section}} 

\ld{let me try to break this apart and relate it to the spectrum}

The test collection approach to \ac{IR} requires the creation of queries, documents and relevance judgments---any or all of these components can in theory be automatically created or generated. Prior works have mostly considered the partial automatization of the query component.

\paragraph{Mostly Automatic Assessment Strategies}
A diverse range of manual test collections are widely used in the \ac{IR} community. However, the manual effort associated with their creation is staggering. Several approaches to semi-automatic support in test collection creation have been proposed, including the use of active learning for annotation and evaluation metrics that correct for the resulting biases~\cite[\textsl{--inter alia}]{cormack1998efficient,jayasinghe2014improving,yilmaz2008simple,zhang2018evaluating}. While these significantly reduce the cost, they still rely on manual annotations. 

\ld{Note to self: these should be spelled out more.}


\paragraph{Fully Automatic Test Collections}

Approaches for fully automatic benchmark creation have also been discussed in the community. \citet{berendsen2013pseudo} and \citet{azzopardi2007building} suggest to simulate artificial queries by selecting terms that maximize the probability of discriminating between the relevant and non-relevant document set. An open question is how to ensure that these queries represent realistic information needs.

Alternatively, semi-structured articles can be exploited, such as using anchor text \citep{asadi2011pseudo}, metadata of scientific article sections \citep{berendsen2012generating}, categories in the Open Directory Project \citep{beitzel2003using},  glosses in Freebase \citep{dalvi2015automatic} or infoboxes \cite{kasneci2009yago,hewlett2016wikireading}.

The  Wikimarks approach \citep{dietz2022wikimarks} derives queries from the title and heading structure of Wikipedia articles, for which passages under the heading are taken as relevant. This approach has also been applied to aspect-based summarization \cite{hayashi2021wikiasp}, and text segmentation \cite{arnold2019sector}.

A question is how well automatic assessments would agree with manual assessments. To this end, a study on the correlation of leaderboards on the TREC CAR data  found a very high rank correlation \citep{dietz2020humans}. 


==> body/related-work/rw-automatic-evaluation.tex <==
\subsection{Automatic evaluation and Query Performance Prediction}

\ld{Suggestion: Reduce the text to talk about QPP in the context of evaluation and in the context of automation.  I personally would prefer less use of acronyms.}
A related body of work concerns the \ac{QPP}, which is defined as the task of evaluating the performance of an \ac{IR} system, in the absence of human-made relevance judgements~\cite{Hauff2010,CarmelYomtov2010}. \ac{QPP} has proven to be effective on several tasks related to the \ac{IR}  evaluation and system development, such as pathological query discovering~\cite{CarmelYomtov2010}, model selection~\cite{CarmelYomtov2010,ThomasScholerEtAl2017}, and query rewriting~\cite{ThomasScholerEtAl2017,ScellsAzzopardiEtAl2018}.
%In particular, it has been used to diagnose pathological queries~\cite{CarmelYomtov2010}, but also to carry out model selection~\cite{CarmelYomtov2010,ThomasScholerEtAl2017}, as a signal in rank fusion algorithms~\cite{Roitman2018c}, for query rewriting, and query formulation selection ~\cite{ThomasScholerEtAl2017,ScellsAzzopardiEtAl2018}.
While \ac{QPP} does not focus directly on the prediction of the relevance for single documents, several works already demonstrated the effectiveness of \acp{LLM} in predicting the performance of a query. 
To provide some examples, BERT-QPP, as proposed by \citet{ArabzadehKhodabakhshEtAl2021}, exploits \acp{LLM} by fine-tuning a BERT model to predict if top-$k$ retrieved documents in response to the query are relevant. On the same note, \citet{DattaMacavaneyEtAl2022} and \citet{ChenHeEtAl2022}, use \acp{LLM} to predict the relevance of the documents retrieved in response to a group of queries.
%\acp{LLM} have been used for automatic evaluation by the means of \ac{QPP} also in specific \ac{IR} tasks where \ac{LLM} have proven particularly effective. For example, \citet{ArabzadehSeifikarEtAl2022} apply \acp{LLM} to predict the performance in the \ac{CS} domain. In particular, Authors of \cite{ArabzadehSeifikarEtAl2022} use BERT to define a cluster of documents, and, by measuring the cluster's internal cohesion determine if the user's question was understood by the system. In a similar effort, \cite{RoitmanEreraEtAl2019} propose a predictor for \ac{QA} meant to determine if the answer provided to the user contains relevant information.
In this regard, our proposal for automatic assessment of the documents using \ac{LLM} not only would provide benefits to a number of downstream tasks, such as \ac{QPP}, but its effectiveness has already been partially shown and is supported by flourishing literature in the \ac{QPP} domain~\cite{ArabzadehKhodabakhshEtAl2021,DattaMacavaneyEtAl2022,ChenHeEtAl2022,ArabzadehSeifikarEtAl2022}.

==> body/related-work/rw-human-assessment.tex <==
\subsection{Human-made assessment}


==> deprecated/contribution.tex <==
\section{Left-overs}

\ld{This text is a victim of my reorganization. I picked up thoughts not already discussed elsewhere and merged them in the text above. Please double check if I was missing something important}

\subsection{Using LLMs to Generate Annotations and Label Automatically}

\ld{The way the text is currently written, it would fit better in the Introduction. It would help to first introduce the spectrum, then we can refer to it across related work, experiments, future, and conclusion }

Potential uses of LLMs to annotate documents, extract snippets, summarize and, in the end, annotate documents for relevance. If this can be made to work reliably, it opens up many opportunities for evaluation. For example, the LLM can be used directly to evaluate the output of other large language models (for example in summarization). 

Assessments can arise from different sources, with different levels of quality and collection costs as follows. 

\begin{itemize}
    \item Human assessors or, in the enterprise scenario, final users. This scenario, at the current time, is the most expansive, but also likely to produce high-quality annotations.
    \item Human assessors aided by mild automatic support systems (e.g. remove redundancy, encourage consistency)
    \item Half of the judgments are produced by human assessors and half of the judgments are produced automatically.
    \item Automatic annotation of a collection, which is verified and corrected by human intervention.
    \item At some point even a fully automatic assessment.
\end{itemize}


An additional axis describes the type of annotations. Typically an annotation is a graded relevance judgment, but for example in EXAM \cite{sander2021exam}, humans are used for generating questions instead. This can be generalized by asking human assessors for something different than traditional annotation while some Machine Learning (ML) converts the human responses into relevance assessments. This follows the paradigm of Competence Partitioning of Human-Machine-Collaboration where humans and machines are performing tasks they are best at (not vice versa).

\ld{moved to dangers} One concern is that fully automatic assessment with LLMs can be very expensive, which is also the reason why we consider the application of LLMs as part of the retrieval process. In such a case, we could reduce the cost by considering a teacher-student training paradigm (knowledge distillation) in which a large and expensive LLM is used to train a smaller model that is less expensive to run.

\ld{the truth part is moved to dangers} Not all IR tasks focus on topics. For example, one may want to search for podcasts where two or more people interact or with a particular style.
Another issue is regarding truth. For example, finding a podcast for the query “does lemon cure cancer?” that talks about healing cancer with lemon might be on topic. Nevertheless, it is unlikely to be factually correct, and therefore not relevant to correctly answering the information need. To overcome this issue, assessors have to access external information to determine the trustworthiness of a source, or the truthfulness of a document.
In a similar way, we can assume our LLM is used as an oracle that accesses external facts, verified by humans. To properly support different tasks, human intervention can be plugged into the collection and annotation of additional facts, to define relevance.

\ld{moved to dangers} There are open questions for the special case of 100\%-machine / 0\%human. How is this ranking evaluation different from being an approach that produces a ranking? (circularity problem).
We can use multiple LLMs, possibly based on different rationales, such that it is possible to define an inter-annotation systems agreement, in which different systems are used to verify if there is an agreement between each other. An alternative approach is to endow the evaluation with additional information about relevant facts/questions/nuggets that the system (under evaluation) does not have access to. 

\ld{moved to dangers}It is yet to be understood what are the risks associated with such technology: it is likely that in the next few years, we will assist in a substantial increase in the usage of LLMs to replace human annotators. Nevertheless, a similar change in terms of data collection paradigm was observed with the increased use of crowd assessor. Up to that moment, annotations were typically made by in-house experts. Then, such annotation tasks were delegated to crowd workers, with a substantial decrease in terms of quality of the annotation, compensated by a huge increase in annotated data. 
It is a concern that machine-annotated assessments might degrade the quality, while dramatically increasing the number of annotations available.

\ld{merged to dangers} The Cranfield paradigm~\cite{Voorhees2001} is based on simplifying assumptions that make manual evaluation feasible: \textit{1)} independence of queries; \textit{2)} independence of relevance of documents; \textit{3)} Relevance is static (and not changing in time). 
Recently, the field is diverging from this paradigm, for example with TREC CAR and TREC CAST/iKAT where the information needs are developing as the user learns more about the domain. The TREC Evaluation of CAST describes a tree of connected information needs, where one conversation takes a path through the tree. The Human-Machine evaluation paradigm might make it feasible to assess more connected (and hence, realistic) definitions of relevance.


\gd{possibly here or at the end of section 2, it would be good to compare the different methods to collect judgments by their \$ cost, e.g., cost of \$0.05 for an AI to judge;  \$0.50 for the crowd; \$5.00 for NIST assessors?}

==> deprecated/experimental-evaluation/charlie.tex <==

To complement the experiments reported in Section~\ref{sec:evaluation}, in this section we report an experiment to fully re-judge submissions to a single evaluation exercise, the passage ranking task of the TREC~2021 Deep Learning Track~\cite{craswell2022overview}. Unlike the experiments reported in Section~\ref{sec:evaluation}, which focused on binary relevance, we attempt to adhere as closely as possible to the methodology used in the track itself, including the use of graded judgments.

\subsection{Methodology}

\citet{craswell2022overview} provide full details of the passage ranking task of the TREC~2021 Deep Learning Track (TREC-DL~2021). TREC-DL~2021 track participants submitted 63~experimental runs, with each run comprising up to 1000~ranked passages for 200~test queries. These runs were pooled, and 53~queries were judged by assessors using a combination of methods, including active learning~\cite{trec2021,AbualsaudGhelaniEtAl2018}. This generated a total of 10,828~judgments on a 4-point scale: ``Perfectly relevant'' $\succ$ ``Highly relevant'' $\succ$ ``Related'' $\succ$ ``Irrelevant''.

We re-judged this pool using the GPT-3.5 {\tt text-davinci-003} language model, as accessed through Open AI's~API in February~2023. Consistent with a classification task---and consistent with the GPT-3.5 experiments reported in Section~\ref{sec:evaluation}---we set the \emph{temperature} parameter to~0, but otherwise default parameters and settings. %Recall that since {\tt text-davinci-003} was trained on data gathered before~2022 and not deployed until November~2022, it was not trained on TREC-DL~2021 judgments nor was it used in a ranker for that task. In this sense, the LLM is independent of the queries and runs.

Since our prompt is relatively long, we provide it online.%
\footnote{\url{https://plg.uwaterloo.ca/~claclark/trec2021_DL_prompt.txt}}
%\footnote{\url{https://anonymous.4open.science/r/SIGIR-2023-F35A/trec2021_DL_prompt.txt}}
The prompt is inspired by a prompt appearing in \citet{Ferraretto23}: importantly---and different from the prompt in Figure~\ref{fig:prompt}---it leverages few-shot learning by listing  multiple \emph{examples} illustrating different levels of relevance for different queries. We provide one example each for ``Perfectly relevant'', ``Highly relevant'', and ``Related''; we provide two examples for ``Irrelevant'', with one providing a judged ``Irrelevant'' passage, and the other providing an unrelated passage from the pool. These examples were chosen arbitrarily from the pool, based on the TREC judgments. We also used the term ``Relevant'' in the prompt, instead of ``Related'', since ``Related'' is a non-standard label for relevance judgments; in preliminary experiments, the LLM would sometimes return ``Relevant'' unprompted. Using this prompt, judgments cost around USD~1~cent each. For this experiment we spent a total of USD~111.90, including a small number of duplicate requests due to failures and other issues. To provide a basis for comparison, \citet{ClarkeVtyurinaEtAl2021} report spending USD~25 cents per human label on a judgment task of similar scope---with a single-page ``prompt'' and no training of assessors.

\subsection{Results}

\begin{figure}[t]%
\centering%
\includegraphics[width=0.8\linewidth, keepaspectratio]{figures/map.png}
%\hspace{20pt}%
%\kern-3em%
\includegraphics[width=0.8\linewidth, keepaspectratio]{figures/ndcg.png}%
\mycaption{Scatter plots comparing the performance of TREC 2021 Deep Learning Track passage ranking runs using official, human judgments and unofficial, LLM judgments, with MAP (top) and NDCG@10 (bottom). A point represents the performance of a single experimental run avg. over all queries.}%
\label{fig:DL}%
\end{figure}

\input{tables/DL-confusion-single-column.tex}
%\input{tables/DL-confusion.tex} %%same table content as above but spread over two tables


Table~\ref{tbl:DL} provides a summary of the results. We provide a summary for both the full 4-point relevance scale and a binary relevance scale, which follows the TREC-DL~2021 convention for computing binary measures such as MAP. This convention maps ``Perfectly relevant'' and ``Highly relevant'' to ``Relevant'', and maps ``Relevant'' and ``Irrelevant'' to ``Not relevant''. Whereas for Table~\ref{tbl:dl21}, in order to compare results with YouChat, we followed the more usual convention of treating all grades except ``Irrelevant'' as relevant. On the binary judgments of Table~\ref{tbl:DL}, Cohen's~$\kappa = 0.26$,  a level of agreement that is conventionally described as ``fair''. To provide a basis for comparison, \citet{cormack1998efficient} report results corresponding to a Cohen's~$\kappa = 0.52$ on a similar experiment comparing two types of human judgments, a level of agreement conventionally described as ``moderate''. 
We applied the LLM~judgments to compute standard evaluation measures on the runs submitted to TREC-DL~2021, with the results shown in Figure~\ref{fig:DL}. Kendall's~$\tau$ values show the correlation between system rankings. To provide a basis for comparison, \citet{Voorhees2000} report a Kendall's~$\tau = .90$ for MAP on a similar experiment comparing two types of human judgments. Nonetheless, the top run under the official judgments remains the top run under the LLM~judgments. 
% Don't use any of the text below.-- CHARLIE
%Hypothetically, if we were employing LLM~judgments to choose the best submitted retrieval approach, it would choose the same as the human judgments, at least in this case.
%This would mean that, at least on this single hypothetical experiment, if we were to replace human assessors with LLMs, we would choose the same retrieval approach for deployment.
We find that measures computed under the LLM~judgments are less sensitive than measures computed under human judgments.
Sensitivity (or ``discriminative power'') measures the ability of an evaluation method to recognize a significant difference between retrieval approaches~\cite{sakai06,ymt18,ClarkeVtyurinaEtAl2021,FaggioliFerro2021}.
To compute sensitivity, we take all pairs of experimental runs and compute a paired t-test between them.
A pair with~$p < 0.05$ is considered to be \emph{distinguished}~\cite{ymt18}, with sensitivity defined as $\frac{\textit{\# of distinguished pairs}}{\textit{total pairs}}$.
Since we do not correct for the multiple comparisons problem, some of the distinguished pairs may not represent actual significant differences. 
%Nonetheless, sensitivity provides a measure of the overall ability of an evaluation method to recognize significant differences~\cite{sakai06,ymt18,crowdpref},  
%A pair with~$p < 0.05$ is considered to be \emph{distinguished}, with sensitivity defined as $\frac{\textit{\# of distinguished pairs}}{\textit{total pairs}}$.
%
Under human judgments 72\% of systems are distinguished under MAP (74\% under NDCG@10). In contrast, under GPT-3.5 judgments only 65\% are distinguished (69\% under NDCG@10). 
%Here no Bonferroni correction was performed, which would lower the number of distinguished pairs proportionally.

% Of course, because there is no Bonferroni or other correction, some of the distinguished pairs may not represent actual significant differences, but the relative number of distinguished pairs provides an indication as to the evaluation method's ability to recognize significant differences. On this experiment, human judgments provide greater sensitivity as shown in Table~\ref{tbl:sensitivity}.

% \begin{table}
% \caption{Sensitivity analysis on TREC-DL 2021.}
% \label{tbl:sensitivity}
% \begin{tabular}{@{}lcc@{}}
% \toprule
% \textbf{Sensitivity} & \textbf{MAP} & \textbf{NDCG@10} \\
% \midrule
% Human judgments & 0.72 & 0.74 \\
% GPT-3.5 judgments   & 0.65 & 0.69 \\
% \bottomrule
% \end{tabular}
% \end{table}











==> deprecated/experimental-evaluation/experimental-methodology.tex <==
To provide a preliminary assessment of today's LLMs' capability for relevance judgments, we conduct an empirical comparison between human and LLM assessors. This comparison includes two LLMs (GPT-3.5 and YouChat), two test collections (the TREC-8 ad~hoc retrieval task~\cite{VoorheesHarman1999} and the TREC~2021 Deep Learning track~\cite{craswell2022overview}), two types of judgments (binary and graded), and two tailored prompts. The experiments were conducted in January and February~2023.

\subsection{Methodology}

Our experiments are not meant to be exhaustive but rather to explore where LLMs~(dis-)agree with manual relevance judgments.

\paragraph{LLMs}
We selected two~LLMs for our experiments: GPT-3.5, more specifically \texttt{\small text-davinci-003}%
\footnote{\url{https://spiresdigital.com/new-gpt-3-model-text-davinci-003}}
accessed via OpenAI's~API,%
\footnote{\url{https://platform.openai.com/docs/api-reference/introduction}}
and YouChat. GPT-3.5~is an established standard model for many applications and thus serves as a natural baseline, while, shortly after \mbox{OpenAI's} release of ChatGPT, YouChat has been one of the first~LLMs to be fully integrated with a commercial search engine%
\footnote{\url{https://you.com}.}
for the task of generating a new kind of search engine result page~(SERP) on which a generated text summarizes the top-$k$ search results ($k \lesssim 5$) in a query-biased way with numbered in-text references to $k$~results listed as ``blue links'' below the summary.

\paragraph{Test Collections}
We base our experiments on (i)~the ad hoc retrieval task of TREC-8~\cite{VoorheesHarman1999} and (ii)~the passage retrieval task of the TREC~2021 Deep Learning track (TREC-DL~2021)~\cite{craswell2022overview}. Both collections have many relevance judgments but also have contrasting properties. TREC-DL~2021 comprises short documents and queries phrased as questions, while TREC-8 comprises much longer, complete documents, with detailed descriptions of information needs, explicitly stating what is (not) considered relevant. As an experimental corpus, TREC-DL~2021 provides the additional benefit that its release date (second half of~2021) falls after the time that training data was crawled for GPT-3.5~(up to June~2021) but falls before the release of GPT-3.5 itself (November~2022).%
\footnote{\url{https://platform.openai.com/docs/models/overview}}
Hence, GPT-3.5 has not been trained on TREC-DL~2021 relevance judgments, nor has it been used as a component in any system participating in TREC-DL~2021.

\paragraph{Judgment Sampling}
We sampled $n=1000$ topic--document pairs each from the relevance judgments files of TREC-8 and TREC-DL~2021 but due to a limited scalability when using YouChat, for some experiments had to restrict ourselves to $100$~random samples per relevance grade (binary for TREC-8, graded for TREC-DL~2021). 

\paragraph{Prompts}
We used two simple and straightforward prompts for the two collections (cf.~Figure~\ref{fig:prompt}) but explicitly did not spend time on optimizing the prompts (so-called ``prompt engineering'') to keep the prompts straightforward and to the point as a first baseline. Formulating and studying better prompts is left for future work.

\paragraph{Answer Parsing}
We recorded the models' generated answers and mapped them to binary relevance judgments. As for GPT-3.5, the prompts and setting $\textit{temperature}=0$ were sufficient to constrain the model to emit only one of the requested relevance grades. As for YouChat, the answers were more verbose but rather homogeneous. With only two exceptions, they started with ``The document~/~passage is \emph{relevant}~[\ldots]'' or with ``The document~/~passage is \emph{not relevant}~[\ldots]'' and were thus straightforward to parse.

\begin{figure}
\begin{greyQuote}
\small
Instruction: You are an expert assessor making TREC relevance judgments. You will be given a TREC topic and a portion of a document. If any part of the document is relevant to the topic, answer ``Yes''. If not, answer ``No''. Remember that the TREC relevance condition states that a document is relevant to a topic if it contains information that is helpful in satisfying the user's information need described by the topic. A document is judged relevant if it contains information that is on-topic and of potential value to the user.

\vspace{1ex}
Topic: \texttt{\{topic\}}\newline
Document: \texttt{\{document\}}\newline
Relevant?
\end{greyQuote}
\vspace{0.25cm}
\begin{greyQuote}
\small
Instruction: Indicate if the passage is relevant for the question.

\vspace{1ex}
Question: \texttt{\{question\}}\newline
Passage: \texttt{\{passage\}}
\end{greyQuote}
\mycaption{Prompts used in our experiments on TREC-8 (top) and TREC-DL~2021 (bottom). At the placeholders \texttt{\{topic\}}, \texttt{\{document\}}, \texttt{\{question\}}, and \texttt{\{passage\}}, the actually sampled pairs are included.}
\label{fig:prompt}
\end{figure}

==> deprecated/experimental-evaluation/experimental-results.tex <==
\subsection{Results}

Table~\ref{tbl:trec8} shows the results for TREC-8. We observe a clear divide according to the relevance label. For documents judged as non-relevant by human assessors, GPT-3.5 generates the same judgment in~90\% of the cases. In contrast though, for the documents judged as relevant by human assessors, this agreement drops to~47\%. Likewise, YouChat has judged 74\%~of the non-relevant documents correctly, but this agreement drops even more to~33\% for the relevant ones.

\input{tables/charlie-results.tex}

Interestingly though, the results on TREC-DL~2021 in Table~\ref{tbl:dl21} show an opposite trend for YouChat: the higher the relevance grade, the more YouChat is in line with the human assessors. For~96 out of 100~question--passage pairs that TREC assessors judged as highly relevant (i.e.,~grade~3), YouChat agreed with the assessors. In contrast, for the non-relevant question--passage pairs, the agreement seems more or less random: YouChat only agrees with the manual assessments on~42 of the 100~pairs. Similarly, on TREC-DL~2021, GPT-3.5 seems to have problems with the middle grades of~1 and~2.

\input{tables/martin-results.tex}

We thus hypothesize that human assessors may use subtle details to distinguish `somewhat relevant' from `probably non-relevant documents' in the binary case that are not captured by the~LLMs and similarly that also the ``differences'' that human assessors use to decide some difficult 1-or-0~cases on a 3--0-scale might rather still be too subtle to be recognizable for the~LLMs.

==> deprecated/experimental-evaluation/experimental-setting.tex <==
%\subsection{Experimental Setting}
%\gf{Description of the experimental setting: collections, \acp{LLM} considered}
%\gf{[TODO: this is Dagstuhl. What is the new setting?] To assess the feasibility of the proposed approaches, next steps would include an experimental comparison of the different \ac{CHM} paradigms. This should include multiple test collections (e.g., TREC-8 and TREC Deep Learning), multiple types of judgments (e.g., binary, graded, preference), and multiple models (e.g., GPT-2, GPT-3, chatGPT, etc.). Comparison between human-generated judgments and machine-generated judgments may be performed both using inter-assessor agreement metrics as well as IR system ranking correlation methods.}


==> deprecated/notes.tex <==
\section*{Todos}


%Noriko: Related work on human assessment
%Ian ?
%Charlie: Experiments
%Benno: Comparing Experiments (+ most urgent task)  -- Spectrum figure
%Martin: Manually done experiments + collect auto-judgments + analysis of results
%Matthias: Introduction + Experiments
%Evangelos + Gianluca + Laura: defining additional experiments modelling Human in the Loop
%Gianluca: Related Work Crowdsourcing, Human/machine assisted judgments
%Guglielmo: Introduction + Paper Organization + If help is Experiment
%Guglielmo: Document the experimental protocol. (Ian: test for missed documents and non-relevant documents near the top)
%Claudia: Related Work
%Laura: Related Work + Everything else
%EVERYONE: Paragraph for the Future
%?  Describes the range from human to machine | spectrum is difficult


@Noriko Kando and  @Ian Soboroff: notes about manual judgement\\

\noindent @Benno Stein:  Laura's and Claudia's notes to table 2 and describe it within the section OPEN ISSUES, FORESEEABLE RISKS, AND OPPORTUNITIES\\

\noindent @Charles Clarke and @Martin Potthast  notes about the methodology in section 5.1 and 5.2  \\

\noindent @Evangelos Kanoulas @Henning Wachsmuth @Gianluca @Matthias Hagen: notes on your opinion on the Discussion section: what are the possibilities and limitations of using LLMs for automatic assessment? \\

\noindent @dietz, @Claudia Hauff @Guglielmo uniform and integrate notes.\\




\section*{Prompts (for humans)}
\subsection*{Blog posts}
http://www.faculty.ucr.edu/~eschwitz/SchwitzPapers/GPT-3-Dennett-230201a.htm

https://ehudreiter.com/2023/01/23/chatgpt-data-to-text/

 https://www.merlin.tech/what-will-ediscovery-lawyers-do-after-chatgpt/

 https://www.washingtonpost.com/technology/2019/07/25/social-media-companies-are-outsourcing-their-dirty-work-philippines-generation-workers-is-paying-price/

Relevant tweet: \url{https://twitter.com/ylecun/status/1617254676428111872}

\subsection*{Papers}
https://arxiv.org/abs/2302.00093
https://arxiv.org/abs/2301.07597


\subsection*{Experiments}

\url{https://docs.google.com/spreadsheets/d/1n5vPT0pMG786RQC_1FD4k0RdQEhmCeqZQ0ZrOcU988E/edit}

\noindent\url{https://docs.google.com/document/d/1iom2pS5CX9UvPWxHw2mtOA7eUUgIkVIXDBZntfB-N0A/edit}


BIBLIO NOT FIXABLE
Can we get rid of TREC assessors? Using Mechanical Turk for relevance assessment.
The Aslib Cranfield Research Project on the Comparative Efficiency of Indexing Systems
FIRE ’22: Proceedings of the 14th Annual Meeting of the Forum for Information Retrieval Evaluation
Relevance reconsidered
Relevance and information behavior
Literature survey of statistical, deep and reinforcement learning in natural language processing
Overview of TREC 2021


==> deprecated/related-work/related-work.tex <==
\section{Background and Related Work (max 1.5 pages)}

\label{subsubsec:evaluation-gaps}

\input{body/related-work/rw-human-assessment.tex}
\input{body/related-work/rw-crowd-hybrid-assessment.tex}
\input{body/related-work/rw-automatic-evaluation.tex}
\input{body/related-work/rw-automatic-assessment.tex}

\input{body/related-work/rw-automatic-assessment-LD.tex}

\progressMarker{End of page 5}


==> deprecated/related-work/rw-automatic-assessment-LD.tex <==


\subsection{Automatic Test Collections \ld{already merged into the new RW section}} 

\ld{let me try to break this apart and relate it to the spectrum}

The test collection approach to \ac{IR} requires the creation of queries, documents and relevance judgments---any or all of these components can in theory be automatically created or generated. Prior works have mostly considered the partial automatization of the query component.

\paragraph{Mostly Automatic Assessment Strategies}
A diverse range of manual test collections are widely used in the \ac{IR} community. However, the manual effort associated with their creation is staggering. Several approaches to semi-automatic support in test collection creation have been proposed, including the use of active learning for annotation and evaluation metrics that correct for the resulting biases~\cite[\textsl{--inter alia}]{cormack1998efficient,jayasinghe2014improving,yilmaz2008simple,zhang2018evaluating}. While these significantly reduce the cost, they still rely on manual annotations. 

\ld{Note to self: these should be spelled out more.}


\paragraph{Fully Automatic Test Collections}

Approaches for fully automatic benchmark creation have also been discussed in the community. \citet{berendsen2013pseudo} and \citet{azzopardi2007building} suggest to simulate artificial queries by selecting terms that maximize the probability of discriminating between the relevant and non-relevant document set. An open question is how to ensure that these queries represent realistic information needs.

Alternatively, semi-structured articles can be exploited, such as using anchor text \citep{asadi2011pseudo}, metadata of scientific article sections \citep{berendsen2012generating}, categories in the Open Directory Project \citep{beitzel2003using},  glosses in Freebase \citep{dalvi2015automatic} or infoboxes \cite{kasneci2009yago,hewlett2016wikireading}.

The  Wikimarks approach \citep{dietz2022wikimarks} derives queries from the title and heading structure of Wikipedia articles, for which passages under the heading are taken as relevant. This approach has also been applied to aspect-based summarization \cite{hayashi2021wikiasp}, and text segmentation \cite{arnold2019sector}.

A question is how well automatic assessments would agree with manual assessments. To this end, a study on the correlation of leaderboards on the TREC CAR data  found a very high rank correlation~\citep{dietz2020humans}. 


==> deprecated/related-work/rw-automatic-evaluation.tex <==
\subsection{Automatic evaluation and Query Performance Prediction}

\ld{Suggestion: Reduce the text to talk about QPP in the context of evaluation and in the context of automation.  I personally would prefer less use of acronyms.}
A related body of work concerns the \ac{QPP}, which is defined as the task of evaluating the performance of an \ac{IR} system, in the absence of human-made relevance judgements~\cite{Hauff2010,CarmelYomtov2010}. \ac{QPP} has proven to be effective on several tasks related to the \ac{IR}  evaluation and system development, such as pathological query discovering~\cite{CarmelYomtov2010}, model selection~\cite{CarmelYomtov2010,ThomasScholerEtAl2017}, and query rewriting~\cite{ThomasScholerEtAl2017,ScellsAzzopardiEtAl2018}.
%In particular, it has been used to diagnose pathological queries~\cite{CarmelYomtov2010}, but also to carry out model selection~\cite{CarmelYomtov2010,ThomasScholerEtAl2017}, as a signal in rank fusion algorithms~\cite{Roitman2018c}, for query rewriting, and query formulation selection ~\cite{ThomasScholerEtAl2017,ScellsAzzopardiEtAl2018}.
While \ac{QPP} does not focus directly on the prediction of the relevance for single documents, several works already demonstrated the effectiveness of \acp{LLM} in predicting the performance of a query. 
To provide some examples, BERT-QPP, as proposed by \citet{ArabzadehKhodabakhshEtAl2021}, exploits \acp{LLM} by fine-tuning a BERT model to predict if top-$k$ retrieved documents in response to the query are relevant. On the same note, \citet{DattaMacavaneyEtAl2022} and \citet{ChenHeEtAl2022}, use \acp{LLM} to predict the relevance of the documents retrieved in response to a group of queries.
%\acp{LLM} have been used for automatic evaluation by the means of \ac{QPP} also in specific \ac{IR} tasks where \ac{LLM} have proven particularly effective. For example, \citet{ArabzadehSeifikarEtAl2022} apply \acp{LLM} to predict the performance in the \ac{CS} domain. In particular, Authors of \cite{ArabzadehSeifikarEtAl2022} use BERT to define a cluster of documents, and, by measuring the cluster's internal cohesion determine if the user's question was understood by the system. In a similar effort, \cite{RoitmanEreraEtAl2019} propose a predictor for \ac{QA} meant to determine if the answer provided to the user contains relevant information.
In this regard, our proposal for automatic assessment of the documents using \ac{LLM} not only would provide benefits to a number of downstream tasks, such as \ac{QPP}, but its effectiveness has already been partially shown and is supported by flourishing literature in the \ac{QPP} domain~\cite{ArabzadehKhodabakhshEtAl2021,DattaMacavaneyEtAl2022,ChenHeEtAl2022,ArabzadehSeifikarEtAl2022}.

==> deprecated/related-work/rw-crowd-hybrid-assessment.tex <==

\paragraph{Crowdsourcing} As document collections kept growing in size, the ratio of documents that could practically be judged by human assessors kept getting smaller. This triggered the research community to look for ways to scale-up the collection of human-generated relevance judgments.
% 
Around 2010, research looking at replacing trained human assessors leveraging micro-task crowdsourcing started to appear \cite{alonso2009can}. In the last 10 years, the community has been looking at research questions related to the reliability of crowdsourced relevance judgments \cite{BlancoHalpinEtAl2011} as well as at questions related to cost and quality management \cite{maddalena2016crowdsourcing}. The increase in possible scale and accessibility of work power usually comes with a decrease in reliability, often due to the complicated interaction of crowd workers and task requesters \cite{nouri:2020}.
% 
The current understanding based on research findings is that crowdsourcing relevance judgments is a viable solution to scaling up the collection of labels and an alternative approach to traditional relevance judgments performed by trained human assessors. This is true as long as quality control mechanisms are put in place and the domain is accessible to non-experts~\cite{tamine2017impact}. Quality control mechanisms may include label aggregation methods \cite{sheshadri2013square}, task design strategies \cite{AlonsoBaezayates2011,kazai2013analysis}, and crowd worker selection strategies \cite{gadiraju2019crowd}.
% 
Recent research has looked at how to support crowd workers in judging relevance by presenting them with extra information (e.g., machine-generated metadata) that can increase their judgment efficiency \cite{xu2023role}.

==> deprecated/related-work/rw-human-assessment.tex <==
\subsection{Human-made assessment}


==> ictir23-automatic-relevance-judgments-part1.tex <==
\section{Introduction} \label{sec:introduction}

Evaluation is very important to the information retrieval~(IR) community and the difficulty of proper evaluation setups is well-known and often discussed (e.g.,~\cite{Saracevic1995,Jarvelin2009,Fuhr2018,Sakai2021}). Many long-standing evaluation campaigns like~TREC, NTCIR, CLEF, or~FIRE~\cite{FIRE2022,Harman1993,Kando1999,Braschler2001} trace their roots back to the Cranfield paradigm~\cite{Cleverdon1960}, which relies on test collections that consist of (i)~a document corpus, (ii)~a set of information needs or topics, and (iii)~relevance judgments for documents on the topics. Critically, according to the Cranfield paradigm, human assessors are needed for the relevance judgments---a time-intensive and costly procedure.%
\footnote{As a concrete example, for the 50~topics in the TREC-8 Ad Hoc track~\cite{VoorheesHarman1999}, 129~participating systems led to more than 86,000~pooled documents to judge, requiring more than 700~assessor hours at a cost of about~USD~15,000.}

\begin{figure}
\begin{greyQuote}
\colorbox{white}{
\includegraphics{human-logo} \small Dear\,LLM, can\,you\,assist\,us\,with\,relevance\,judgments?}

\ \,\includegraphics{chatgpt-logo} \small Yes, I can certainly provide assistance with relevance judgments. Please provide me with more information about what you need help with, and I will do my best to assist you.

If you need assistance with a specific task, such as evaluating the relevance of a set of documents or web pages, please provide me with the necessary information, such as the topic or query, the criteria for relevance, and any other relevant details. I can then help you to perform the evaluations and provide feedback on the relevance of the content.
\end{greyQuote}
\mycaption{Asking ChatGPT for assistance on February~15, 2023.}
\label{fig:ask-chatgpt}
\end{figure}

However, over the past decades, in~IR more and more tasks have been delegated to machines that were traditionally performed by humans, starting with indexing and retrieval. While the idea of automatically generated judgments has been considered before~\cite{soboroff2001ranking}, it has not found widespread use in the IR~community. Other previous ideas to minimize the cost of collecting relevance judgments include judging text nuggets instead of documents~\cite{pavlu2012ir}, using crowdworkers~\cite{alonso2009can,BlancoHalpinEtAl2011} (though this comes with its own set of problems~\cite{maddalena2016crowdsourcing}), cleverly selecting which documents to judge~\cite{CarteretteAllanEtAl2006,jayasinghe2014improving}, constructing test collections from Wikipedia~\cite{dietz2022wikimarks}, or automating parts of the judgment process via a QA~system~\cite{sander2021exam}.

Figure~\ref{fig:ask-chatgpt} shows the response of ChatGPT%
\footnote{\url{https://chat.openai.com/chat}}
when asked whether it can assist with relevance judgments. ChatGPT suggests that it is able to carry out relevance judgments, but it is unclear how well such judgments align with those made by human annotators. In this perspectives paper, we explore whether we are on the verge of being able to delegate relevance judgments to machines---either fully or partially---by employing large language models~(LLMs). 
We aim to provide a balanced view on this contentious question by presenting both consenting and dissenting voices in the scientific debate surrounding the use of~LLMs for relevance judgments. Although a variety of document modalities exist (audio, video, images, text), we here focus on text-based test collections. The consolidated methodology for assessing the relevance of textual documents, which dates back to the Cranfield paradigm, enables us to carry out a grounded comparison between~LLMs and human assessors. While the technology might not be ready yet to provide fully automatic relevance judgments, we argue that LLMs are already able to help humans in relevance assessment---to various extents. To model the range of automation options, we propose and discuss a spectrum of collaboration between humans and~LLMs (cf.~Table~\ref{table-perspective-collaboration}): from manual judgments, the current setup, to fully automated judgments that are carried out solely by~LLMs as a potential future option.

Some of the spectrum's scenarios have already been studied (cf.~Section~\ref{sec:related-work}), while others are currently emerging. We describe risks as well as open questions that require further research and we conduct a pilot feasibility experiment where we assess how well judgments generated by~LLMs agree with humans, including an analysis of LLM-specific caveats. To conclude our paper, we provide two opposing perspectives---for and against the use of~LLMs as relevance ``assessors''---, as well as a compromise between them. All of the perspectives are informed by our analyses of the literature, our pilot experimental evidence, and our experience as IR~researchers.

==> ictir23-automatic-relevance-judgments-part2.tex <==
\section{Related Work} \label{sec:related-work}

Following the Cranfield paradigm, a test collection-based approach to IR~evaluation requires documents, queries, and relevance judgments for query--document pairs. The traditional approach to acquire relevance judgments is to hire human assessors. However, the judgment effort is staggering, leading to a range of approaches to assist the assessors or to automate tedious tasks. Below, we describe existing approaches and relate them to our human--machine collaboration spectrum (cf.~Table~\ref{table-perspective-collaboration}).

\subsection{Human Judgment}
As document collections kept growing in size, the ratio of documents that could practically be judged by human assessors kept getting smaller. This triggered the IR~community to look for ways to scale-up human-generated relevance judgments. Around~2010, replacing trained human assessors by micro-task crowdsourcing became an option~\cite{alonso2009can} so that the community started to study the reliability of crowdsourced relevance judgments~\cite{BlancoHalpinEtAl2011} and questions related to cost and quality management~\cite{maddalena2016crowdsourcing}.

The workforce increased via crowdsourcing usually comes with a decreased reliability, often due to the complicated interactions between crowdworkers and task requesters \cite{nouri:2020}. Still, before the advent of large language models, several studies showed that crowdsourcing is a viable alternative to scale-up relevance judgments compared to the ``classic'' hiring of trained human assessors---as long as the domain is accessible to non-experts and quality control mechanisms are put in place~\cite{tamine2017impact}. Quality control mechanisms may include label aggregation methods~\cite{sheshadri2013square}, task design strategies~\cite{AlonsoBaezayates2011,kazai2013analysis}, and crowdworker selection strategies~\cite{gadiraju2019crowd}.

Some studies have tried to increase the judgment efficiency of crowdworkers by adding machine-generated information (e.g., metadata)~\cite{xu2023role} but recent findings suggest that LLMs~alone are even better at several text annotation tasks than crowdworkers~\cite{GilardiAlizadehEtAl2023}.

\subsection{Human Verification and AI Assistance}
In this scenario, humans partially relinquish control over which documents will be assessed or how machine assessments will be derived but humans remain in control of defining relevance.

For example, some studies suggest to adjust evaluation metrics to be able to deal with incomplete judgments (e.g.,~\cite{yilmaz2008simple,froebe:2023}). This way, judgment costs can be reduced by reducing the number of assessments needed for evaluating retrieval systems.

Alternatively, \citet{keikha2014evaluating} suggest to automatically transfer manual relevance judgments in the context of passage retrieval: any unjudged passage that has a high similarity to a judged passage will inherit the judged passage's relevance label on a given topic. In the original setup, the authors used ROUGE as the similarity measure but also ``modern'' alternatives like BertScore~\cite{zhang2019bertscore} could be tried---as transferring relevance judgments between corpora without proper similarity checking is problematic~\cite{froebe:2022}.

Other ideas for semi-automatic relevance judgments are active learning~\cite{cormack1998efficient} (e.g., human assessors only label documents for which an automatic relevance assessment has a low confidence) or to automatically identify potentially relevant documents that only manual runs would contribute to the pool~\cite{jayasinghe2014improving}---in order to construct low-bias reusable test collections. 

Instead of asking humans for relevance assessments on query--document pairs, \citet{sander2021exam} suggest to ask humans for (exam) questions related to a query~/~topic that should be answerable from the content of a relevant document. The more of the manually formulated questions an automatic question-answering system can answer, the more relevant a to-be-judged document is---captured by the authors' proposed EXAM answerability metric. Similar ideas have also been used successfully in other labeling tasks~\cite{eyal2019question,deutsch2021towards,huang2020knowledge}.

\subsection{Fully Automated Test Collections}
Inspired by ideas from evaluating aspect-based summarization \cite{hayashi2021wikiasp} or text segmentation~ \cite{ArnoldSchneiderEtAl2019}, the Wikimarks approach~\cite{dietz2022wikimarks} aims to automatically create queries and judgments for a test collection. The title and subheadings of Wikipedia articles are used to formulate queries and the passage below the title~/~heading is assumed to be relevant for the respective query---without actual human judgments. Similar distant supervision-style approaches to acquire relevance assessments for ``artificial'' queries exploit other facets of human-authored (semi-structured) documents: anchor text~\cite{AsadiMetzlerEtAl2011}, metadata of scientific articles~\cite{BerendsenTsagkiasEtAl2012}, categories in the Open Directory Project~\cite{BeitzelJensenEtAl2003}, glosses in Freebase~\cite{dalvi2015automatic}, or infoboxes~\cite{kasneci2009yago,hewlett2016wikireading}.

Also for the task of query performance prediction~(QPP)~\cite{Hauff2010,CarmelYomtov2010}, the goal is to estimate retrieval effectiveness (i.e., the ability to return relevant results) without having manual relevance judgments---often even without knowing the actual retrieval results. While some recent studies effectively used~LLMs in QPP~scenarios~\cite{ArabzadehKhodabakhshEtAl2021,DattaMacavaneyEtAl2022,ChenHeEtAl2022,ArabzadehSeifikarEtAl2022,FaggioliFerroEtAl2023}, an open question still is how well LLM-based relevance assessments agree with manual assessments. A study on the leaderboards of the TREC CAR track found a very high rank correlation~\cite{dietz2020humans} and some preliminary evidence seems to indicate that LLMs~can replace human assessors in several NLP~tasks~\cite{ZhuZhangEtAl2023}---with a high variance in the quality of the annotations, though---, but \citet{MacAvaneySoldaini2023} found that automatic relevance judgments may correlate poorly with human assessments. Still, system leaderboards obtained from the automatic relevance judgments were comparable to those based on manual assessments.

==> ictir23-automatic-relevance-judgments-part3.tex <==
\section{Spectrum of Human--Machine Collaboration} \label{sec:spectrum}

\input{tables/table-perspective-collaboration}

To discuss potential capabilities of~LLMs in the context of relevance judgments, we devise a human--machine collaboration spectrum with different levels of ``labor division'' between humans and LLMs (cf.\ Table~\ref{table-perspective-collaboration} for an overview). At one end, humans manually judge without any LLM~interaction, while at the other end, LLMs replace humans completely. In between, LLMs assist humans at various degrees of interdependence.

\paragraph{Human Judgment} On this end of the spectrum, humans manually decide what is relevant without being influenced by an~LLM. In reality, of course, humans are still supported by basic features of a judgment interface. Such features might still be based on heuristics that do not require any form of automatic training~/~feedback. For instance, humans may define so-called scan terms to be highlighted in a text, they may limit viewing the pool of documents that have already been judged, or they may order documents by similarity so that it is easier to assign the same relevance label to similar documents. This end of the spectrum thus represents the status quo, where humans are considered the only reliable judges.

\paragraph{AI Assistance} More advanced assistance can come in many forms. For example, an~LLM may generate a summary of a to-be-judged document so that a human assessor can more efficiently make a judgment based on the compressed representation. Another approach could be to manually define information nuggets that are relevant (e.g., exam questions~/~answers~\cite{sander2021exam}) and to then train an~LLM to automatically indicate how many test nuggets are contained in a to-be-judged document (e.g., via a QA~system). This directly implies questions towards improving the human--machine collaboration: How to employ~LLMs, as well as other AI~tools, to aid human assessors in devising reliable judgments while enhancing the efficiency of the process? What are tasks that can be taken over by~LLMs (e.g., document summarization or keyphrase extraction)? 

\paragraph{Human Verification} For each document to judge, a first-pass judgment of an~LLM is automatically produced as a suggestion along with a generated rationale. We consider this to be a \textit{human-in-the-loop} approach: one or more~LLMs provide their relevance judgment and humans verify them. In most cases, the humans might not have to intervene at all but they might still be required in challenging situations where the~LLM has low confidence.

An idea could also follow the `preference testing' paradigm~\cite{windsor1994preference}: two~LLMs each generate a judgment, and a human will select the better one---intervening only in case of disagreement between the~LLMs. Still, in the scenario of human verification, humans make the ultimate decision wherever needed. A concern then could be that some bias of the~LLMs might affect the final relevance judgments, as humans might not be able to recognize all biases. Related questions that we wish to raise within the community are: What sub-tasks of the judgment process require human input (e.g., prompt engineering~\cite{ZhouMuresanuEtAl2022,SorensenRobinsonEtAl22}---for now) and for what tasks or judgments should human assessors \emph{not} be replaced by machines?

\paragraph{Fully Automated} If LLMs were able to reliably assess relevance, they could completely replace humans in the judgment process. A fully automatic judgment system might be as good as humans in producing high-quality relevance judgments (for a specific corpus~/~domain) but automatic judgments might even surpass humans in terms of quality, which raises the follow-up issue of how to detect that.
A question that our community ought to investigate thus is: How can and should humans be replaced entirely by~LLMs in the judgment process? Indeed, one could go as far as asking whether generative~LLMs can and should be used to create complete test collections by generating documents~/~passages, as well as queries~/~conversations and relevance judgments. 

\medskip
A central aspect to be investigated is where on this four-level human--machine collaboration spectrum we actually obtain the ideal relevance judgments at the best cost. At this point, humans perform tasks that humans are good at, while machines perform tasks that machines are good at---often referred to as competence partitioning~\cite{hancock2013task,flemisch2016shared}: a task is assigned to either a human or a machine, depending on who is better suited. Note that in our current version of the spectrum, we still (optimistically) show \emph{balanced} competence partitioning as part of `AI assistance'.

==> ictir23-automatic-relevance-judgments-part4.tex <==
\section{Open Issues and Opportunities} \label{sec:dangers}

In this section, we identify several issues that arise when LLMs~are used during relevance judgment tasks. We discuss open questions, risks we foresee, as well as opportunities to move beyond the currently accepted retrieval evaluation paradigms.

\subsection{LLM Judgment Cost and Quality}
It is currently unclear what the benefits and risks of~LLMs for relevance judgments are. This situation is similar to the time when crowdsourced judgments became possible. Until about 10--15~years ago, judgments typically came from (trained) in-house experts but then suddenly could be delegated to cheaper crowdworkers resulting in an increased amount of financially feasible judgments---but at a substantially decreased quality~\cite{HalveyVillaEtAl2015} so that quality-assurance methods had to be developed~\cite{DanielKucherbaevEtAl2018}. With LLMs, history may somewhat repeat itself. Based on current pricing models, the inference costs per LLM~judgment can be much lower than for crowdsourcing (cf.\ the estimates in the column `Cost' of Table~\ref{table-perspective-substitution}) so that again an increase in the amount of financially feasible judgments (from~LLMs) is very likely. Still, the effect with respect to judgment quality is unclear---even improvements are possible---and can only be clarified~/~controlled by conducting respective studies and developing LLM-specific quality estimation and assurance methods.

\input{tables/table-perspective-substitution}

The pressing question is: What is the effectiveness of LLM-based judgment (support)? In Table~\ref{table-perspective-substitution}, we depict our current understanding by distinguishing four assessor types (user, expert, crowdworker, and LLM) and four judgment tasks: preference (which of two documents is more relevant?), binary (is this document relevant?), graded (how relevant is this document?), and explained (justify a judgment). The table entries indicate potential substitutions in the sense that similar abilities of~LLMs hint at a replaceability of respective assessors (e.g., LLMs instead of crowdworkers for binary judgments). Still, the table cannot fully clarify the role of~LLMs as we are still in the early stages of development and simply do not know the eventual capabilities: \bsplus\ and \bsdot\ in the `LLM'~row should thus be interpreted with these current uncertainties in mind.

To align their judgments with humans, LLMs could be fine-tuned by observing human relevance assessors or they might use an active learning strategy~\cite{SharmaKaushik2017,YuChungEtAl2022,SeungminDonghyunEtAl2022}. For instance, an~LLM could start with mild suggestions to a human assessor on how relevant a document is and could then continuously learn from the actual judgments of the assessor to improve its own suggestions.

\subsection{Human Verification}
\paragraph{Using Multiple LLMs as Assessors}
While hiring multiple human relevance assessors with different backgrounds usually is very easy and potentially occurring judgment disagreements are not unresolvable~\cite{FerranteFerroEtAl2017}, many~LLMs are trained on very similar web corpora which may yield highly correlated judgments of not yet known quality or bias. A possible solution to obtain less correlated~LLMs is to train or fine-tune them on different data (e.g., subcorpora). Fine-tuning on different user types could even yield ``personalized'' models~\cite{YoonYun2017,JaechOstendorf18,WelchGuEtAl2022} that might enable automatic judgments according to specific user groups' perspectives on relevance.

\paragraph{Truthfulness \& Misinformation}
An important aspect of relevance judgments is factuality. For a question like ``do lemons cure cancer?'', some top-ranked document may indeed suggest lemons as a treatment for cancer. While topically matching, the content is unlikely to be factually correct and the document should therefore be judged as non-relevant. Trained human assessors may very well be able to determine the trustworthiness of a document and, at least to some extent, the truthfulness. But the ability of~LLMs to do so is quite unclear and probably also depends on the characteristics of the training data that often are not disclosed. This raises at least two questions: Can we automatically assess the reliability and factuality of LLM-generated relevance judgments? Can we identify the textual training sources underlying an LLM's~judgment and can we verify that they are represented accurately?

Going forward, it will also be vital to be able to distinguish human-generated from automatically generated sources, especially in contexts such as journalism where correctness is critical.

\paragraph{Bias}
\citet{BenderGebruEtAl2021} highlight limitations of~LLMs and identify bias as a severe risk. As LLMs~are intrinsically biased \cite{BastaCostajussaEtAl2019,KuritaVyasEtAl2019,HutchinsonPrabhakaran2020}, such bias may also be reflected in LLMs' relevance judgments. For example, an LLM might be prone to consider scientific documents as relevant, while documents written in informal language are perceived as less relevant. The IR~community should focus on finding ways to evaluate~LLMs in terms of judgment bias, i.e., to analyze to what extent the intrinsic bias actually affects evaluations using LLM-supported~/~LLM-based relevance judgments.

\paragraph{Faithful Reasoning.}
LLMs often generate text that contains inaccurate or false information (i.e., they confabulate or ``hallucinate'') and usually do so in an affirmative manner that makes it difficult for humans to even suspect errors. In response, the NLP~community is exploring a new research direction called ``faithful reasoning''~\cite{CreswellShanahan2022}. This approach aims to generate text that is less opaque, also describing explicitly the step-by-step reasoning, or the ``chain of thoughts''~\cite{LyuHavaldarEtAl2023}. A similar idea of ``reasoned'' automatic relevance judgments might be an interesting IR~research direction.

\paragraph{Explaining Relevance to LLMs}
Judgment guidelines often provide a comprehensive overview of what constitutes a relevant document in what scenario---most famously, Google's search quality evaluator guidelines have more than 170~pages.%
\footnote{\url{https://guidelines.raterhub.com/searchqualityevaluatorguidelines.pdf}}
Still, it is open how such guidelines should be ``translated'' to prompt~LLMs. In addition, relevance may go beyond topical relevance~\cite{Saracevic1996}. For instance, a certain style may be required or the desired information should allure users from certain communities or cultures with different belief systems. We do not yet know to what extent LLMs~are capable of assessing such different variations of relevance so that human intervention might still play a central role when taking document aspects into account that may not yet be easily discernable by~LLMs.

\subsection{Fully Automated}
\paragraph{LLM-based Evaluation of LLM-based Systems}
In the fully automated scenario, a circulatory problem can arise: Why not use a good LLM-based relevance assessor as an actual approach to produce a ranking? However, in practical settings, we expect LLMs~used for ranking to be much smaller (more cost effective, lower latency, etc.; e.g., via knowledge distillation) than LLMs~used for judging. In addition, the judging~LLMs may have additional information about relevant facts~/~questions~/~nuggets that a ranker does not know, and, as assessment latency might not be an issue, different (more complex) judging~LLMs may even be combined in an ensemble.

\paragraph{Moving beyond Cranfield}
Given limited time or monetary budgets, retrieval evaluations based on manual judgments are often only feasible due to ``standard'' simplifying assumptions. For example, document collections are assumed to be static, small sets of queries~/~topics are assumed to suffice, and a document's relevance is assumed to not change (definitely a simplification~\cite{Schamber1994,Voorhees2000}) and to be independent of other documents. If LLMs would produce reliable relevance judgments with little human verification effort, many of the simplifying assumptions could be relaxed. For example, in search sessions or in the TREC CAsT track~\cite{DaltonXiong2020,DaltonXiong2020b},%
\footnote{TREC CAsT is a shared task that aims at evaluating conversational agents and thus provides information needs in the form of multi-turn conversations, each containing several utterances that a user might pose to an agent.}
information needs are changing over the course of a session or a conversation as the user learns more about a topic. Collaborative human--machine relevance judgment might help to scale-up evaluations using such more comprehensive and thus more realistic notions of relevance.

\paragraph{Moving beyond Human.} \label{sec:beyond-human}
Finally, at one end of our proposed spectrum, machines may surpass humans in the relevance judgment task. This phenomenon has already been witnessed in a variety of NLP~tasks, such as scientific abstract classification~\cite{GohCaiEtAl2020} or sentiment detection~\cite{WeismayerPezenkaEtAl2018}. Humans are likely to make mistakes when judging relevance and are limited by time. It is conceivable that LLMs with sufficient monetary funds will be capable of providing a larger number of more consistent judgments. However, if we use human-annotated data as a gold standard, we will not be able to detect when LLMs~surpass human judgment quality as we then will have reached the limit of measurement.

==> ictir23-automatic-relevance-judgments-part5.tex <==
\section{Preliminary Assessment} \label{sec:evaluation}

To provide a preliminary assessment of today's LLMs' capability for relevance judgments, we conduct an empirical comparison between human and LLM assessors. This comparison includes two LLMs (GPT-3.5 and YouChat), two test collections (the TREC-8 ad~hoc retrieval task~\cite{VoorheesHarman1999} and the TREC~2021 Deep Learning track~\cite{craswell2022overview}), two types of judgments (binary and graded), and two tailored prompts. The experiments were conducted in January and February~2023.

\subsection{Methodology}

Our experiments are not meant to be exhaustive but rather to explore where LLMs~(dis-)agree with manual relevance judgments.

\paragraph{LLMs}
We selected two~LLMs for our experiments: GPT-3.5, more specifically \texttt{\small text-davinci-003}%
\footnote{\url{https://spiresdigital.com/new-gpt-3-model-text-davinci-003}}
accessed via OpenAI's~API,%
\footnote{\url{https://platform.openai.com/docs/api-reference/introduction}}
and YouChat. GPT-3.5~is an established standard model for many applications and thus serves as a natural baseline, while, shortly after \mbox{OpenAI's} release of ChatGPT, YouChat has been one of the first~LLMs to be fully integrated with a commercial search engine%
\footnote{\url{https://you.com}.}
for the task of generating a new kind of search engine result page~(SERP) on which a generated text summarizes the top-$k$ search results ($k \lesssim 5$) in a query-biased way with numbered in-text references to $k$~results listed as ``blue links'' below the summary.

\paragraph{Test Collections}
We base our experiments on (i)~the ad hoc retrieval task of TREC-8~\cite{VoorheesHarman1999} and (ii)~the passage retrieval task of the TREC~2021 Deep Learning track (TREC-DL~2021)~\cite{craswell2022overview}. Both collections have many relevance judgments but also have contrasting properties. TREC-DL~2021 comprises short documents and queries phrased as questions, while TREC-8 comprises much longer, complete documents, with detailed descriptions of information needs, explicitly stating what is (not) considered relevant. As an experimental corpus, TREC-DL~2021 provides the additional benefit that its release date (second half of~2021) falls after the time that training data was crawled for GPT-3.5~(up to June~2021) but falls before the release of GPT-3.5 itself (November~2022).%
\footnote{\url{https://platform.openai.com/docs/models/overview}}
Hence, GPT-3.5 has not been trained on TREC-DL~2021 relevance judgments, nor has it been used as a component in any system participating in TREC-DL~2021.

\paragraph{Judgment Sampling}
We sampled $n=1000$ topic--document pairs each from the relevance judgments files of TREC-8 and TREC-DL~2021 but due to a limited scalability when using YouChat, for some experiments had to restrict ourselves to $100$~random samples per relevance grade (binary for TREC-8, graded for TREC-DL~2021). 

\paragraph{Prompts}
We used two simple and straightforward prompts for the two collections (cf.~Figure~\ref{fig:prompt}) but explicitly did not spend time on optimizing the prompts (so-called ``prompt engineering'') to keep the prompts straightforward and to the point as a first baseline. Formulating and studying better prompts is left for future work.

\paragraph{Answer Parsing}
We recorded the models' generated answers and mapped them to binary relevance judgments. As for GPT-3.5, the prompts and setting $\textit{temperature}=0$ were sufficient to constrain the model to emit only one of the requested relevance grades. As for YouChat, the answers were more verbose but rather homogeneous. With only two exceptions, they started with ``The document~/~passage is \emph{relevant}~[\ldots]'' or with ``The document~/~passage is \emph{not relevant}~[\ldots]'' and were thus straightforward to parse.

\begin{figure}
\begin{greyQuote}
\small
Instruction: You are an expert assessor making TREC relevance judgments. You will be given a TREC topic and a portion of a document. If any part of the document is relevant to the topic, answer ``Yes''. If not, answer ``No''. Remember that the TREC relevance condition states that a document is relevant to a topic if it contains information that is helpful in satisfying the user's information need described by the topic. A document is judged relevant if it contains information that is on-topic and of potential value to the user.

\vspace{1ex}
Topic: \texttt{\{topic\}}\newline
Document: \texttt{\{document\}}\newline
Relevant?
\end{greyQuote}
\vspace{0.25cm}
\begin{greyQuote}
\small
Instruction: Indicate if the passage is relevant for the question.

\vspace{1ex}
Question: \texttt{\{question\}}\newline
Passage: \texttt{\{passage\}}
\end{greyQuote}
\mycaption{Prompts used in our experiments on TREC-8 (top) and TREC-DL~2021 (bottom). At the placeholders \texttt{\{topic\}}, \texttt{\{document\}}, \texttt{\{question\}}, and \texttt{\{passage\}}, the actually sampled pairs are included.}
\label{fig:prompt}
\end{figure}

\subsection{Results}

Table~\ref{tbl:trec8} shows the results for TREC-8. We observe a clear divide according to the relevance label. For documents judged as non-relevant by human assessors, GPT-3.5 generates the same judgment in~90\% of the cases. In contrast though, for the documents judged as relevant by human assessors, this agreement drops to~47\%. Likewise, YouChat has judged 74\%~of the non-relevant documents correctly, but this agreement drops even more to~33\% for the relevant ones.

\input{tables/charlie-results.tex}

Interestingly though, the results on TREC-DL~2021 in Table~\ref{tbl:dl21} show an opposite trend for YouChat: the higher the relevance grade, the more YouChat is in line with the human assessors. For~96 out of 100~question--passage pairs that TREC assessors judged as highly relevant (i.e.,~grade~3), YouChat agreed with the assessors. In contrast, for the non-relevant question--passage pairs, the agreement seems more or less random: YouChat only agrees with the manual assessments on~42 of the 100~pairs. Similarly, on TREC-DL~2021, GPT-3.5 seems to have problems with the middle grades of~1 and~2.

\input{tables/martin-results.tex}

We thus hypothesize that human assessors may use subtle details to distinguish `somewhat relevant' from `probably non-relevant documents' in the binary case that are not captured by the~LLMs and similarly that also the ``differences'' that human assessors use to decide some difficult 1-or-0~cases on a 3--0-scale might rather still be too subtle to be recognizable for the~LLMs.

==> ictir23-automatic-relevance-judgments-part6.tex <==
\section{Re-Judging TREC 2021 Deep Learning} \label{sec:charlie}

To complement the experiments from Section~\ref{sec:evaluation}, we now re-evaluate submissions to the passage ranking task of the TREC~2021 Deep Learning track~\cite{craswell2022overview} (TREC-DL~2021) using LLM-based judgments but adhering as closely as possible to the methodology used in the track itself~\cite{craswell2022overview}, including the use of graded judgments.

\subsection{Methodology}

The participants of TREC-DL~2021 submitted 63~runs, each comprising up to 1000~ranked passages for 200~questions. These runs were pooled, and the results for 53~questions were judged by assessors using a combination of methods, including active learning~\cite{trec2021,AbualsaudGhelaniEtAl2018}. This generated a total of 10,828~judgments on a 4-point scale: `perfectly relevant' $\succ$ `highly relevant' $\succ$ `relevant' (named `related' in the track) $\succ$ `non-relevant' (named `irrelevant' in the track).

We re-judged this pool using the GPT-3.5 \texttt{\small text-davinci-003} language model, as accessed through Open AI's~API in February~2023. Consistent with a classification task---and with our GPT-3.5~experiments reported in Section~\ref{sec:evaluation}---, we set $\textit{temperature}=0$ and otherwise use default parameters and settings.

Our relatively long prompt%
\footnote{Available at: \url{https://plg.uwaterloo.ca/~claclark/trec2021_DL_prompt.txt}}
is inspired by a prompt of \citet{Ferraretto23}: importantly---and different from the prompt in Figure~\ref{fig:prompt}---it leverages few-shot learning by listing  multiple \emph{examples} illustrating different levels of relevance for different questions. We provide one example each for `perfectly relevant', `highly relevant', and `relevant', and we provide two examples for `non-relevant', with one providing a judged `non-relevant' passage, and the other providing an unrelated passage from the pool. These examples were chosen arbitrarily from the pool, based on the TREC~judgments. We also used the term `relevant' in the prompt, instead of `related', since `related' is a non-standard label for relevance judgments; in preliminary experiments, the LLM would sometimes return `relevant' unprompted. Using this prompt, each judgment did cost about USD~0.01---we spent a total of USD~111.90, including a small number of duplicate requests due to failures and other issues. In comparison, \citet{ClarkeVtyurinaEtAl2021} report spending USD~0.25 per human judgment on a task of similar scope---with a single-page ``prompt'' and no training of assessors.

\subsection{Results}

\begin{figure}[t]%
\centering%
\includegraphics[width=0.8\linewidth, keepaspectratio]{figures/map.png}

\vspace{4ex}
\includegraphics[width=0.8\linewidth, keepaspectratio]{figures/ndcg.png}%
\mycaption{Scatter plots of the effectiveness of TREC-DL~2021 runs (MAP (top) and NDCG@10 (bottom)) according to the track's human judgments and our LLM-based judgments. A point represents a single run averaged over all questions.}%
\label{fig:DL}%
\end{figure}

\input{tables/DL-confusion-single-column.tex}
%\input{tables/DL-confusion.tex} %%same table content as above but spread over two tables


Table~\ref{tbl:DL} shows the ``agreement'' on the full 4-point relevance scale and on a binarized relevance scale---following the TREC-DL~2021 convention, we map `perfectly relevant' and `highly relevant' to `relevant', and `relevant' and `non-relevant' to `non-relevant'. On the binarized judgments the Cohen's~$\kappa$ is~$0.26$, which indicates a `fair' level of agreement. Note that on a similar experiment with two types of human judgments,  \citet{cormack1998efficient} report a Cohen's~$\kappa$ of~$0.52$ (`moderate' agreement). 

Compared to the system rankings using the official judgments, using the LLM~judgments to compute standard evaluation measures for the runs submitted to TREC-DL~2021 yields the correlations and Kendall's~$\tau$ values shown in Figure~\ref{fig:DL}. Note that the top run under the official judgments remains the top run under the LLM~judgments. For comparison, \citet{Voorhees2000} report a Kendall's~$\tau = .90$ for MAP on a similar experiment with two types of human judgments.

We find that measures computed under the LLM~judgments are less sensitive than measures computed under human judgments. Sensitivity (or ``discriminative power'') measures the ability of an evaluation method to recognize a significant difference between retrieval approaches~\cite{sakai06,ymt18,ClarkeVtyurinaEtAl2021,FaggioliFerro2021}. To compute sensitivity, we take all pairs of submitted runs and compute a paired t-test between them. Here, we consider a pair with~$p < 0.05$ as \emph{distinguished}~\cite{ymt18} and define sensitivity as $\frac{\textit{\# of distinguished pairs}}{\textit{total pairs}}$. Since we do not correct for the multiple comparisons problem, some of the distinguished pairs may not represent actual significant differences. With human judgments, 72\%~of the pairs are distinguished under~MAP (74\%~under NDCG@10). In contrast, with GPT-3.5 judgments, only 65\%~are distinguished under~MAP (69\% under~NDCG@10). 








==> ictir23-automatic-relevance-judgments-part7.tex <==
\section{Perspectives for the Future} \label{sec:future}

As this is a perspectives paper, we provide two opposing perspectives on the use of~LLMs for automatic relevance judgments---for and against---and a third compromise perspective.


\subsection{In Favor of Using LLMs for Judgments}

In addition to providing a judgment of relevance, LLMs are able to produce a natural language explanation \textit{why} a certain document is relevant or not to a topic~\cite{Ferraretto23}. Such AI-generated explanations may be used to assist human assessors in relevance judgments, particularly non-experts like crowdworkers. This setup may lead to better quality judgments as compared to the unsupported crowd. While LLM-generated labels and explanations may lead to an overreliance of human assessors
, human assessors may serve as a quality control mechanism for the LLM. Furthermore, they serve as a feedback loop for the LLM to continuously improve its judgments. 
Our pilot experiments demonstrate that it is feasible for LLMs to indicate when a document is likely not relevant. We might therefore let human annotators assess (a)~first those documents that are deemed relevant by~LLMs, or (b)~a subsample of documents from those considered relevant by the LLM, as an LLM can be run at scale. Thereby, we envision the use of LLMs to reduce annotation cost/time when creating high-quality IR~evaluation collections.

It is noteworthy that LLMs may be better at providing fair and consistent judgments than humans. They can judge the relevance of documents without being affected by documents they have seen before, and with no boredom or tiredness effects. They are likely to assess conceptually similar documents the same way. Furthermore, they will often have seen much more information on a specific topic than most humans.
%
Another advantage of today's LLMs is their inherent ability to process and generate text in many different languages. For multilingual corpora (which often appear in industrial settings) the assessment is typically restricted to a small subset of languages due to the limited availability of assessors. With LLMs being part of the assessment tool, this limitation no longer applies. 
LLMs are not just restricted to one input modality and thus conducting assessments that require the simultaneous consideration of multiple pieces of content (e.g. judging a web page based on the text but also the document's structure, visual cues, embedded video material, etc.) at the same time becomes possible. 
Finally, we note the cost factor---if we are able to judge hundreds of thousands of documents for a relatively small price, we can build much larger and much more complex test collections with regularly updated relevance assessments, in particular in domains that today lack meaningful test collections.

In summary, LLMs can provide explanations, scalability, consistency, and a certain level of quality when performing relevance judgments, underlining the great potential of deploying them as a complement to human assessors in certain judgments task. 



\subsection{Against Using LLMs for Judgments}

While we have given several reasons to believe that we are close to using LLMs for automatic relevance judgment, there are also several concerns that should be addressed by the research community before deploying full-fledged automatic judgment.
The primary concern is that LLMs are not people. IR~measures of effectiveness are ultimately grounded in a human user's relevance judgment.
Relevance is subjective, and changes over time for the same person \cite{mizzaro1997relevance}.
Even if LLMs are increasingly good at mimicking human language in evaluating contents, it is a big leap of faith to fully trust the model's ability to make correct assessments without human verification. Currently, there is no proof that the judgments made by LLMs are grounded in reality.
This raises an essential question: \emph{If the output from an~LLM is indistinguishable from a human-made relevance judgment, is this just a distinction without a difference?} After all, people disagree on relevance and change their opinions over time due to implicit and explicit learning effects. Usually, however, those disagreements do not have an effect on the evaluation unless there are systematic causes~\cite{Voorhees2000,BaileyCSTVY08}.  
To safely adopt LLMs to replace human annotators, the community should examine whether LLM-based relevance judgments may in fact be systematically different from those of real users. Not only do we know this affects the evaluation, but the complexity (or black-box nature) of the model precludes defining systematic bias in any useful way. 
There is a general concern about solely evaluating IR research with relevance assessment: Information retrieval systems are not just result-ranking machines, but are a system that is to assist a human to obtain information. Hence, only the user who consumes the results could tell which ones are useful.
Another concern of applying LLMs as relevance annotators regards the ``circularity'' of the evaluation. Assume we are able to devise an annotation model based on LLMs. The same model could ideally also be used to retrieve and rank documents based on their expected relevance. If the model is used to judge relevance both for annotation and for retrieval, its evaluation would be overinflated, possibly with perfect performance. Vice-versa, models based on widely different rationales (such as BM25 or classical lexical approaches), might be penalized, because of how they estimate document relevance. 
As counter-considerations, we might hypothesize that the model used to label documents for relevance (a)~is highly computationally expensive, making it almost unfeasible to use it as a retrieval system, and/or (b)~has access to more information and facts than the retrieval model. The former holds as long as we do not use the automatic annotator as an expensive re-ranker capable of dealing with just a few documents. The latter, on the other hand, does not solve the problem of the automatic annotation, but simply shifts the problem: Either, the additional facts and information need to be annotated manually; then the human annotator remains essential. Or, the facts can be collected automatically; then we may assume that also a retrieval system could obtain them.

Other concerns arise if we even consider generative models as a replacement for traditional~IR and search. In a plain old search engine, results for a query are ranked according to predicted relevance (ignoring sponsored results and advertising here). Each has a clear source, and each can be inspected directly as an entity separate from the search engine. Moreover, users frequently reformulate queries and try  suggestions from the search engine, in a virtuous cycle wherein the users fulfill or adjust their conceptual information needs. Currently, hardly any of these is possible using LLM-generated responses: The results often are not attributed, rarely can be explored or probed, and are often completely generated. Also, best approaches for prompt engineering are not sufficiently studied, and their effect is more opaque than approaches to query reformulation. LLMs~will not be usable for many information needs until they can attribute sources reliably and can be interrogated systematically. 
Will become available soon.
 
Finally, there are significant socio-technical concerns. Generative AI models can be used to generate fake photos and videos, for extortion purposes and misinformation. They are perceived as stealing the intellectual property. 
Furthermore, LLMs are affected by bias, stereotypical associations~\cite{BastaCostajussaEtAl2019,KuritaVyasEtAl2019}, and adverse sentiments towards specific groups~\cite{HutchinsonPrabhakaran2020}. 
Critically, we cannot assess whether the LLM may have seen information that biases the relevance judgment in an unwanted way, let alone that the company owning the LLM may change it anytime without our knowledge or control. 
As a result, we ourselves as the authors of this perspectives paper disagree on whether, as a profession and considering the ACM's Code of Ethics, we should use generative models in deployed systems {\it at all} until these issues are worked out.



\subsection{A Compromise: Double-checking LLMs and Human--Machine Collaboration}

Our pilot study in Sections~\ref{sec:evaluation} and \ref{sec:charlie} finds a reasonable correlation between highly-trained human assessors and a fully automated LLM, yielding similar leaderboards. This suggests that the technology is promising and deserves further study. The experiment could be implemented to double-check LLM judgments: 
produce fully automated as well as human judgments on a shared judgment pool, then analyze correlations of labels and system rankings,
then decide whether LLM's relevance judgments are good enough to be shared as an alternative test collection with the community. The automatic judgment paradigm should be revealed along with prompts, hyperparameters, and details for reproducibility.
We also suggest to declare which judgment paradigm was chosen when releasing data resources (such as in TREC CAR). At the very least, such automatic judgments could be used to evaluate early prototypes of approaches, for initial judgments for novel tasks, and for large-scale training.


While the discussion is easily dominated by the fully automated evaluation---this is merely an extreme point on our spectrum in Section \ref{sec:spectrum}. The majority of authors do not believe this constitutes the best path towards credible IR research. For example, ``AI Assistance'' is probably the most credible path for LLMs to be incorporated during evaluation. However, it is also the least explored so far.

This calls for more research on innovative ways to use~LLMs for assistance during the judgment process and how to leverage humans for verifying the LLMs'~suggestions. As a community, we should explore how the performance of human assessors changes, when they are shown rationales or chain-of-thoughts that are generated by LLMs. Human assessors often struggle to see a pertinent connection when they are lacking world knowledge. An example of this issue is the task of assessing the relevance of ``diabetes'' for the topic ``child trafficking''. LLMs can generate rationales that can explain such connections. However, it requires a human to realize when such a rationale was hallucinated. Only a human can assess whether the information provided appears true and reliable.

==> ictir23-automatic-relevance-judgments-pre.tex <==
\title{Perspectives on Large Language Models for Relevance Judgment}

\thanks{We thank Ian Soboroff for his ideas, comments, and other contributions.}

\author{Guglielmo Faggioli}
\orcid{https://orcid.org/0000-0002-5070-2049}
\affiliation{%
  \institution{University of Padova}
  \city{}
  \country{}
}
\email{}

\author{Laura Dietz}
\orcid{https://orcid.org/0000-0003-1624-3907}
\affiliation{%
  \institution{University of New Hampshire}
  \city{}
  \country{}
}
\email{}

\author{Charles L.\ A.\ Clarke}
\orcid{https://orcid.org/0000-0001-8178-9194}
\affiliation{%
  \institution{University of Waterloo}
  \city{}
  \country{}
}
\email{}

\author{Gianluca Demartini}
\orcid{https://orcid.org/0000-0002-7311-3693}
\affiliation{%
  \institution{University of Queensland}
  \city{}
  \country{}
}
\email{}

\author{Matthias Hagen}
\orcid{https://orcid.org/0000-0002-9733-2890}
\affiliation{%
  \institution{Friedrich-Schiller-Universit{\"a}t Jena}
  \city{}
  \country{}
}
\email{}

\author{Claudia Hauff}
\orcid{https://orcid.org/0000-0001-9879-6470}
\affiliation{%
  \institution{Spotify}
  \city{}
  \country{}
}
\email{}

\author{Noriko Kando}
\orcid{https://orcid.org/0000-0002-2133-0215}
\affiliation{%
  \institution{National Institute of Informatics (NII)}
  \city{}
  \country{}
}
\email{}

\author{Evangelos Kanoulas}
\orcid{https://orcid.org/0000-0002-8312-0694}
\affiliation{%
  \institution{University of Amsterdam}
  \city{}
  \country{}
}
\email{}

\author{Martin Potthast}
\orcid{https://orcid.org/0000-0003-2451-0665}
\affiliation{%
  \institution{Leipzig University and ScaDS.AI}
  \city{}
  \country{}
}
\email{}

\author{Benno Stein}
\orcid{https://orcid.org/0000-0001-9033-2217}
\affiliation{%
  \institution{Bauhaus-Universit{\"a}t Weimar}
  \city{}
  \country{}
}
\email{}

\author{Henning Wachsmuth}
\orcid{https://orcid.org/0000-0003-2792-621X}
\affiliation{%
  \institution{Leibniz University Hannover}
  \city{}
  \country{}
}
\email{}





\copyrightyear{2023}
\acmYear{2023}
\setcopyright{acmlicensed}\acmConference[ICTIR '23]{Proceedings of the 2023 ACM SIGIR International Conference on the Theory of Information Retrieval}{July 23, 2023}{Taipei, Taiwan}
\acmBooktitle{Proceedings of the 2023 ACM SIGIR International Conference on the Theory of Information Retrieval (ICTIR '23), July 23, 2023, Taipei, Taiwan}
\acmPrice{15.00}
\acmDOI{10.1145/3578337.3605136}
\acmISBN{979-8-4007-0073-6/23/07}

\settopmatter{printacmref=false}


\begin{abstract}
When asked, large language models~(LLMs) like ChatGPT claim that they can assist with relevance judgments but it is not clear whether automated judgments can reliably be used in evaluations of retrieval systems. In this perspectives paper, we discuss possible ways for~LLMs to support relevance judgments along with concerns and issues that arise. We devise a human--machine collaboration spectrum that allows to categorize different relevance judgment strategies, based on how much humans rely on machines. For the extreme point of `fully automated judgments', we further include a pilot experiment on whether LLM-based relevance judgments correlate with judgments from trained human assessors. We conclude the paper by providing opposing perspectives for and against the use of~LLMs for automatic relevance judgments, and a compromise perspective, informed by our analyses of the literature, our preliminary experimental evidence, and our experience as IR~researchers. 
\end{abstract}

\keywords{large language models, relevance judgments, human--machine collaboration, automatic test collections}



\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10002951.10003317.10003359.10003361</concept_id>
<concept_desc>Information systems~Relevance assessment</concept_desc>
<concept_significance>500</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Information systems~Relevance assessment}

\maketitle

\renewcommand{\shortauthors}{Guglielmo Faggioli et al.}


==> ictir23-automatic-relevance-judgments-sum.tex <==
\section{Conclusion} \label{sec:conclusion}

In this paper, we investigated the opportunity that large language models~(LLMs) now may generate relevance judgments automatically. We discussed previous attempts to automate and scale-up the relevance judgment task, and we presented experimental results showing promise in the ability to mimic human relevance assessments with~LLMs. Our findings suggest that, while the path is promising and worthy of being investigated, at the time of writing several reasons prevent~LLMs from being employed as fully automated annotation tools. Nevertheless, there is a spectrum of solutions to employ~LLMs as support for human assessors in a human--machine collaboration. Therefore, we present our perspectives on why and why not the IR~community should employ~LLMs in some way in the evaluation process. Undoubtedly, more research on LLMs~for relevance judgment is to be carried out in the future, for which this paper provides a starting point.

\begin{acks}
This paper is based on discussions during a breakout group at the Dagstuhl Seminar 23031 on ``Frontiers of Information Access Experimentation for Research and Education''~\cite{BauerCarteretteEtAl2023}. We express our gratitude to the Seminar organizers, Christine Bauer, Ben Carterette, Nicola Ferro, and Norbert Fuhr. 

Certain companies and software are identified in this paper in order to specify the experimental procedure adequately. Such identification is not intended to imply recommendation or endorsement of any product or service, nor is it intended to imply that the software or companies identified are necessarily the best available for the purpose.

This material is based upon work supported by the National Science Foundation under
Grant No. 1846017. Any opinions, findings, and conclusions or recommendations expressed in this material
are those of the author(s) and do not necessarily reflect the views of the National Science
Foundation.
\end{acks}

==> notes.tex <==
\section*{Todos}


%Noriko: Related work on human assessment
%Ian ?
%Charlie: Experiments
%Benno: Comparing Experiments (+ most urgent task)  -- Spectrum figure
%Martin: Manually done experiments + collect auto-judgments + analysis of results
%Matthias: Introduction + Experiments
%Evangelos + Gianluca + Laura: defining additional experiments modelling Human in the Loop
%Gianluca: Related Work Crowdsourcing, Human/machine assisted judgments
%Guglielmo: Introduction + Paper Organization + If help is Experiment
%Guglielmo: Document the experimental protocol. (Ian: test for missed documents and non-relevant documents near the top)
%Claudia: Related Work
%Laura: Related Work + Everything else
%EVERYONE: Paragraph for the Future
%?  Describes the range from human to machine | spectrum is difficult


@Noriko Kando and  @Ian Soboroff: notes about manual judgement\\

\noindent @Benno Stein:  Laura's and Claudia's notes to table 2 and describe it within the section OPEN ISSUES, FORESEEABLE RISKS, AND OPPORTUNITIES\\

\noindent @Charles Clarke and @Martin Potthast  notes about the methodology in section 5.1 and 5.2  \\

\noindent @Evangelos Kanoulas @Henning Wachsmuth @Gianluca @Matthias Hagen: notes on your opinion on the Discussion section: what are the possibilities and limitations of using LLMs for automatic assessment? \\

\noindent @dietz, @Claudia Hauff @Guglielmo uniform and integrate notes.\\




\section*{Prompts (for humans)}
\subsection*{Blog posts}
http://www.faculty.ucr.edu/~eschwitz/SchwitzPapers/GPT-3-Dennett-230201a.htm

https://ehudreiter.com/2023/01/23/chatgpt-data-to-text/

 https://www.merlin.tech/what-will-ediscovery-lawyers-do-after-chatgpt/

 https://www.washingtonpost.com/technology/2019/07/25/social-media-companies-are-outsourcing-their-dirty-work-philippines-generation-workers-is-paying-price/

Relevant tweet: \url{https://twitter.com/ylecun/status/1617254676428111872}

\subsection*{Papers}
https://arxiv.org/abs/2302.00093
https://arxiv.org/abs/2301.07597


\subsection*{Experiments}

\url{https://docs.google.com/spreadsheets/d/1n5vPT0pMG786RQC_1FD4k0RdQEhmCeqZQ0ZrOcU988E/edit}

\noindent\url{https://docs.google.com/document/d/1iom2pS5CX9UvPWxHw2mtOA7eUUgIkVIXDBZntfB-N0A/edit}


BIBLIO NOT FIXABLE
Can we get rid of TREC assessors? Using Mechanical Turk for relevance assessment.
The Aslib Cranfield Research Project on the Comparative Efficiency of Indexing Systems
FIRE ’22: Proceedings of the 14th Annual Meeting of the Forum for Information Retrieval Evaluation
Relevance reconsidered
Relevance and information behavior
Literature survey of statistical, deep and reinforcement learning in natural language processing
Overview of TREC 2021


==> tables/DL-confusion.tex <==
\begin{table*}
\caption{Confusion matrices comparing official TREC judgments and unofficial LLM judgments on TREC 2021 Deep Learning Track (DL 2021) query/passage pairs for the passage ranking task. All query--passage pairs judged for the track have been re-judged by the LLM. The matrix on the left compares judgments on all four relevance levels. The matrix on right collapses the relevance levels to two levels, following the DL 2021 convention for computing binary measures.} 
\label{tbl:DL}
\begin{minipage}[t]{0.55\linewidth}
\begin{tabular}[t]{@{}llcccc@{}}
\toprule
\textbf{LLM} & \textbf{Prediction} & \multicolumn{4}{c}{\textbf{TREC-DL~2021 Assessors}}\\
\cmidrule(l@{\tabcolsep}){3-6}
&& Perf.\ rel. & High.\ rel. & Related & Irrelevant \\
\midrule
\multirow{4}{*}{GPT-3.5}
& Perfectly relevant & 250 & 248 &  177 &   87 \\
& Highly relevant    & 360 & 575 &  628 &  370 \\
& Relevant           & 328 & 880 &  798 &  442 \\
& Irrelevant         & 148 & 638 & 1460 & 3439 \\
\bottomrule
\end{tabular}
\end{minipage}%
\hfill%
\begin{minipage}[t]{0.40\linewidth}
\begin{tabular}[t]{@{}llcc@{}}
\toprule
\textbf{LLM} & \textbf{Prediction} & \multicolumn{2}{c}{\textbf{TREC-DL~2021 Assessors}} \\
\cmidrule(l@{\tabcolsep}){3-4}
&& Relevant & Not relevant \\
\midrule
\multirow{2}{*}{GPT-3.5}
& Relevant     & 1433 & 1262 \\
& Not relevant & 1994 & 6139 \\
\bottomrule
\end{tabular}
\end{minipage}
\end{table*}

